Symmetries-enhanced Multi-Agent Reinforcement Learning

Multi-agent reinforcement learning has emerged as a powerful framework for enabling agents to learn complex, coordinated behaviors but faces persistent challenges regarding its generalization, scalability and sample efficiency. Recent advancements have sought to alleviate those issues by embedding intrinsic symmetries of the systems in the policy. Yet, most dynamical systems exhibit little to no symmetries to exploit. This paper presents a novel framework for embedding extrinsic symmetries in multi-agent system dynamics that enables the use of symmetry-enhanced methods to address systems with insufficient intrinsic symmetries, expanding the scope of equivariant learning to a wide variety of MARL problems. Central to our framework is the Group Equivariant Graphormer, a group-modular architecture specifically designed for distributed swarming tasks. Extensive experiments on a swarm of symmetry-breaking quadrotors validate the effectiveness of our approach, showcasing its potential for improved generalization and zero-shot scalability. Our method achieves significant reductions in collision rates and enhances task success rates across a diverse range of scenarios and varying swarm sizes.

==> Extended_version_files/Conclusions_extended.tex <==
\section{Conclusions \& Future Work}

This paper provides the necessary conditions for a MARL problem to exhibit symmetries that can be exploited via equivariant policies. We construct a novel methodology for leveraging extrinsic symmetries, indicated solely by the task, for systems without intrinsic ones and introduce the Group Equivarinat Graphormer, an equivariant neural architecture adaptable to different symmetry groups. The experimental results of our work suggest that embedding extrinsic equivariance in MARL policies is beneficial for the generalization, scalability and sample efficiency. However, a task may be invariant to multiple symmetry groups that are compatible with the manifold but not exhibited by the dynamics. So how do we pick the symmetry group? We select the largest symmetry the reward function would support and leave the symmetry selection strategy for future work.

==> Extended_version_files/DynamicalSystemSymmetries_extended.tex <==
\section{Exploiting Symmetries of Dynamical Systems}\label{section:EquivariantProblem}

 In this section we show that if Problem \ref{eq:prob} exhibits some structural symmetries then the optimal control policy needs to exhibit them as well, leading to sample efficient learning. 

\begin{definition_}
    \label{eq:G-equivariant_problem}
    Consider a real Lie Group $G$, a smooth manifold with group properties satisfying differentiability of group operations. Problem \ref{eq:prob} is $G$-equivariant if, for transitive actions induced by elements of the group $G$ on a vector field $\mathcal{X}$, $\phi:\mathcal{X}\times G \rightarrow \mathcal{X}$ and $ \psi:\mathcal{U}\times G \rightarrow \mathcal{U}$, it satisfies the following properties:
    \begin{enumerate}
        \item \label{eq:G-equivariant_problem1} The objective function is type-0 equivariant (invariant function), i.e . \begin{align*}
            \mathcal{L}(\oplus_{I_N}x_i(t), \oplus_{I_N}u_i(t) )=\mathcal{L}(\oplus_{I_N}\phi_g(x_i(t) ), \oplus_{I_N}\psi_g(u_i(t) ) ),\,\forall g \in G  \end{align*}
        \item \label{eq:G-equivariant_problem2} The robot dynamics are equivariant w.r.t. elements of $G$, i.e. \begin{align*} d\phi_gf(x_i(t),u_i(t)) = f(\phi_g(x_i(t)), \psi_g(u_i(t)),\,\forall g \in G \end{align*} where $d\phi: \mathfrak{X}(\mathcal{X}) \times G\rightarrow \mathfrak{X}(\mathcal{X})$ the differential of the diffeomorphism defining the symmetry.
    \end{enumerate}
\end{definition_}
In RL terminology, this is equivalent to requiring the transition, reward, and observations functions to be invariant under group actions, giving rise to the G-invariant Markov Games.
\begin{remark_}
    Assuming equivariant robot dynamics without dynamical interaction  with tensorial state comprised of type-$0,1,\dots,l$ tensors, the centralized system dynamics described by $\Tilde{f}(x(t),u(t)) = \oplus_{i\in I_N} f(x_i(t),u_i(t))$ are also equivariant, with tensorial state of extended multiplicity $N\cdot mul(l)$ per tensor type $l$. 
\end{remark_}
\begin{theorem_}\label{theorem:equivariant_optimal_control}
    The optimal control policy of the swarm $u^{*}(t)=[\oplus_{\forall i\in I_N} u_i^{*}(t)]$ for the G-equivariant geometric swarming problem, i.e. equation (\ref{eq:prob}) with definition (\ref{eq:G-equivariant_problem}), is equivariant under group actions from elements of $G$.
\end{theorem_}
\begin{proof}
The proof is appended in Appendix I Section \ref{appendix:proofs} of supplemental material.
\end{proof}
Theorem \ref{theorem:equivariant_optimal_control} offers a way to shrink the hypothesis class of the learned controller to that of all G-equivariant functions. This inductive bias usually translates to fewer parameters required and greater sampling efficiency as multiple states $x(t)$ of the G-equivariant problem identified  via the actions of the group $G$, are essentially equivalent, and therefore any G-equivariant policy trained on a dataset $D=\{x^1,x^2,\dots \}$ would generalize to the dataset $\hat{D} = \cup_{\forall g\in G} \{\phi_g(x^1),\phi_g(x^2),\dots\}$ where $D\subseteq \hat{D} \subseteq \cup_{I_N}\mathcal{X}$. Leveraging symmetries is particularly important in multi-agent RL as it is a sampling inefficient learning process.

% \noindent\textbf{Permutation equivariance}: The symmetric group $S_n$ is the group of all permutations of the set.....



\section{When symmetries are broken}\label{section:ArtificialEquivariance}

Section \ref{section:EquivariantProblem} demonstrated why symmetries of dynamical systems are useful. Unfortunately, even though most tasks codified by a reward function exhibit geometric symmetries (condition \ref{eq:G-equivariant_problem1} for G-equivariant problem), most dynamical systems have little to no symmetries to exploit (condition \ref{eq:G-equivariant_problem2} for G-equivariant problem), rendering Theorem \ref{theorem:equivariant_optimal_control} void. To circumvent this issue, we propose embedding the non-equivariant system into an extended dynamical system that is G-equivariant, so that Theorem \ref{theorem:equivariant_optimal_control} stands and the extended learned policy is G-equivariant, and recovering the optimal action for the original non-equivariant dynamical system via the non-equivariant input projective function that guarantees equivalence between the two associated dynamical systems. This way we can provide structure in the learned policy, even if the original dynamical system does not support it. A consequence of this framework is that the structure of the policy is solely constrained by the symmetries that the reward function admits, meaning that any problem can be recast as a G-equivariant problem as long as condition \ref{eq:G-equivariant_problem1} holds and the Lie group G is compatible with the manifold $\mathcal{X}$.

Consider the push-forward smooth map $d_{*}\phi : \mathfrak{X}(\mathcal{X}) \times G\rightarrow \mathfrak{X}(\mathcal{X})$ defined as $d_{*}\phi_g f(x,u):= d\phi_g f (\phi_{g^{-1}}(x),u)$, naturally induced by the diffeomorphism $\phi: G\times \mathcal{X} \rightarrow \mathcal{X}$.
\begin{lemma_}\label{lemma:push_forward}
     The push-forward function $d_{*}\phi$ is a well defined linear group action (automorphism) on the infinite dimensional vector field $\mathfrak{X}(\mathcal{X})$.
\end{lemma_}
\begin{proof}
    We append the proof in Appendix I of supplemental material.
\end{proof}
\begin{theorem_}\label{theorem:equivariant_input_extension}
     Let $f:\mathcal{X}\times \mathcal{U} \rightarrow \mathfrak{X}(\mathcal{X})$ denote a control affine dynamical system on a smooth manifold $\mathcal{X}$ that admits a transitive group action from a compatible Lie group $G$, over an input vector space $\mathcal{U}$. For the extended input vector space $\hat{\mathcal{U}} := span\{d_{*}\phi_{g}f(x,u)\,|\,  u \in \mathcal{U},g \in G\}$, the associated system dynamics  $F:\hat{\mathcal{U}} \times \mathcal{X} \rightarrow \mathfrak{X}(\mathcal{X})$ are equivariant with respect to actions induced by elements of the Lie group $G$.
\end{theorem_}
\begin{proof}
    We append the proof in Appendix I of supplemental material.
\end{proof}
Leveraging theorem \ref{theorem:equivariant_input_extension}, any control affine dynamical system can be embedded in an associated equivariant dynamical system, by extending the input to include the closure of the image of the dynamics under the pushforward operator. The associated dynamics then are $F(x,\hat{u}) := \sum_{j=1}^K d_{*}\phi_{g_j}f(x,u_j)$, for $g_i\in G,u_i\in \mathcal{U},K\in\mathbb{N}, x\in \mathfrak{X}(\mathcal{X}),\hat{u}\in \hat{\mathcal{U}}$. A limiting factor is that, even if the original input space $\mathcal{U}$ is finite dimensional, the extended input vector space $\hat{\mathcal{U}}\subset\mathfrak{X}(\mathcal{X})$ can be infinite dimensional. In practice, for a learning-based controller its dimension is analogous to the dimension of the output features and depends on the complexity of the dynamical system and the selected symmetry group. 
\begin{remark}(\cite{Mahony2020EquivariantST}\label{remark:2}
    The trajectory of a control affine dynamical system $f:\mathcal{X}\times \mathcal{U} \rightarrow \mathfrak{X}(\mathcal{X})$ on a smooth manifold $\mathcal{X}$ is identical to the trajectory of its associated system dynamics $F:\hat{\mathcal{U}} \times \mathcal{X} \rightarrow \mathfrak{X}(\mathcal{X})$, defined in theorem (\ref{theorem:equivariant_input_extension}), if the extended control input is constrained in $\mathcal{U}$, i.e. for some $u(t) \in \mathcal{U}$ $F(x(t),u(t))=f(x(t),u(t))$.
\end{remark}
We can, then, reformulate problem (\ref{eq:prob}) to incorporate artificial symmetries even if the dynamical system does not satisfy the condition \ref{eq:G-equivariant_problem2} of definition \ref{eq:G-equivariant_problem} (only condition \ref{eq:G-equivariant_problem1}) as 
\begin{align}\label{eq:equivariant_problem}
    u^{*}_{0:T,I_N}=& h_{\mathcal{U}}(\argmin_{\hat{u}_{0:T}\in \hat{\mathcal{U}}} \int_{0}^T \mathcal{L}(\oplus_{I_N}x_i(\tau) , \oplus_{I_N} h_\mathcal{U}(\hat{u}_i(\tau))) d\tau) \nonumber\\
    s.t.\quad& \dot{x}_i(t)=F(x_i(t),h_\mathcal{U}(\hat{u}_i(t)))\in \mathfrak{X}(\mathcal{X})\,,\, i\in I_N \nonumber\\
    &\hat{u}_i(t) = \hat{\pi}(o_i(t) \cup x_i(t);\mathcal{O}) \in \hat{\mathcal{U}}
\end{align}
where $h_{\mathcal{U}}:\hat{\mathcal{U}} \rightarrow \mathcal{U}$ a smooth idempotent surjective morphism constraining the extended input to the original input vector space $\mathcal{U} \subset \hat{\mathcal{U}}$.
\begin{proposition}\label{theorem:equivariant_problem}
    Problems (\ref{eq:prob}) and (\ref{eq:equivariant_problem}) are equivalent and, if $\mathcal{L}:\mathcal{X} \rightarrow \mathbb{R}$ is G-invariant, there exists an optimal lifted $\hat{\pi}^{*}:\mathcal{X}^{N} \rightarrow \hat{\mathcal{U}}$ that is G-equivariant.
\end{proposition}
\begin{proof}
   We append the proof in Appendix I of supplemental material.
\end{proof}
From Proposition \ref{theorem:equivariant_problem} there exists a G-equivariant extended optimal policy $\hat{\pi}^{*}: \mathcal{X}^{|\mathcal{N}_i|+1} \rightarrow \hat{\mathcal{U}}$ such that the optimal policy can be decomposed as $\pi^{*}(x_i(t),o_i(t))= h_\mathcal{U} \circ \hat{\pi}^{*} (x_i(t),o_i(t))$. Assuming that the extended input space is finite-dimensional, the universal approximation theorem holds, meaning that the equivariant policy for the associated system can be $\epsilon$-approximated by any G-equivariant neural network $\hat{\pi}_\theta$. Unfortunately, finding the associated equivariant dynamical system is a difficult process, even for systems with simple dynamics, so $h_\mathcal{U}$ is unknown and must also be learned by a neural network $h_\theta$. Without the equivariant analogue system $F$, the policy $\pi_\theta(x_i,o_i)= h_\theta \circ \hat{\pi}_\theta(x_i,o_i) \in \mathcal{U}$ is fitted using data drawn from the original non-equivariant system $f$, whose trajectories identify with $F$, thus there is no guarantee that $\hat{\pi}_\theta \rightarrow \hat{\pi}^{*}$. Still, the existence of $F$ alone guarantees that the compositional policy $\pi_\theta$ is valid, i.e. is a universal approximator of $\pi^{*}$. We demonstrate experimentally in Section \ref{section:experiments} the benefits in generalization and scalability of parametrizing the policy as a composition of a G-equivariant and a non-equivariant neural network.




% If $h_\mathcal{U}$ is not known ...
% If the robot dynamic interaction ...
% \textbf{Picking the symmetry group}...
% Universal approximation ...


==> Extended_version_files/Experiments_extended.tex <==
\section{Experiments} \label{section:experiments}

To evaluate the effectiveness of incorporating artificial symmetries in out MARL scheme, we offer extensive experimentation on swarms of quadrotors. Quadrotors are dynamical systems with few existing geometric symmetries to exploit, namely $S^1$ \cite{10156379}, $SO(2)$ symmetry in downwash models \cite{equivariant_downwash} and $C_2$ symmetries for low level attitude control \cite{10054413}.  \cite{HAMPSEY2023132} proposed an equivariant LQR controller for single-quadrotor trajectory tracking with arbitrary full state symmetries. Full state equivariant Markov Game modeling approaches like \cite{chen2023rm} or \cite{yu2023equivariant} are not applicable due to the lack of symmetries of the dynamical system, as shown in section \ref{section:EquivariantProblem}. Our scheme, presented in sections \ref{section:ArtificialEquivariance}-\ref{section:LieGraphormer}, allows for the embedding of artificial $SE(3)$ symmetry in the distributed controllers, even though the quadrotor model does not exhibit such symmetry, as gravity is invariant to the rotation group. 


\noindent\textbf{Environment}:
Consider a homogeneous swarm of $N$ Crazyflie 2.0 quadrotors with base dynamics
\begin{align*}
    m\cdot \ddot{x}_i &= m\cdot \mathbf{g} + \mathbf{R}_i \mathbf{F}_i \\
    \dot{\omega}_i &= J^{-1}(\tau_i - \omega_i \times (J\cdot\omega_i)) \\
    \dot{\mathbf{R}}_i&= \omega_{i,\times} \mathbf{R}_i
\end{align*}
where $i\in I_N$ the agent tag, $m\in \mathbb{R}_{+}$ denotes the mass, $\ddot{x}_i \in \mathbb{R}^3$ is the acceleration in the world frame, $\mathbf{g}=[0,0,-9.81]^T$ is the gravitational acceleration vector, $\mathbf{R}_i\in SO(3)$ is the rotation matrix from the body frame to the world frame, $\mathbf{F}_i = [0,0,\sum_{1,\dots,4}k_F P_{i,k}^2]^T \in\mathbb{R}^3$ is the total thrust force in the body frame with $P_{i,k}$ the motors' RMPs and $k_F$ constant, $\omega_i \in \mathbb{R}^3$ is the angular velocity in the body frame, $J\in \mathbb{R}^{3 \times 3}$ is the inertia tensor, $\tau_i = \kappa(P_{i,\{1,\dots,4\}}) \in \mathbb{R}^3$ is the total torque in the body frame for some function $\kappa$ that computes the torques induced in the local frame by the motor speeds, and $\omega_{i,\times} \in \mathbb{R}^{3 \times 3}$ is a skew-symmetric matrix associated with the angular acceleration rotated to the world frame. We, further, extend the model to include aerodynamic effects like drag, ground effect and downwash, similarly to \cite{panerati2021learning}, along with appropriate random noise and lag as in \cite{8967695}. For $x_i^d(t)\in \mathbb{R}^3$ desired target position, the state of each robot is defined as $s_i(t) = (x_i(t),\dot{x}_i(t),\mathbf{R}(t),\mathbf{R}(t)\omega(t), x_i^d(t))$ and the observation $o_i(t)=\cup_{j \in \mathcal{N}_i}s_j(t)$, both in the world frame. To facilitate the learning process, instead of the motor speeds we consider the control action to be the normalized motor thrust input $a_i(t)$, i.e. an interpolation between no power and maximum power to the motors. To satisfy the non-negativity of thrusts, the actions $u_i(t)$ are transformed by the policy to $a_i(t)\in [0,1]^4$ with $a_i(t)=(1+\textit{clip}(u_i(t),-1,1))/2$. To learn robust recover policies, the states are randomly initialized. The multi-quadrotor RL environment implementation is based on \cite{huang2023quadswarm}.
One may observe that even the base dynamics of a quadrotor are not $SE(3)$-equivariant, as for any element $(\Bar{x},\Bar{\mathbf{R}})$ of the $SE(3)$ group $$\ddot{\Tilde{x}}_i = \mathbf{g}+m^{-1} \Bar{\mathbf{R}} \mathbf{R}_i [0,0,\sum_{1,\dots,4}k_F P_{i,k}^2]^T \neq \frac{d^2}{d^2t}(\Bar{\mathbf{R}}x_i+\Bar{x})= \Bar{\mathbf{R}} \ddot{x}_i$$, i.e. the gravitional acceleration vector is not rotated by the group action. That means that, even if the rewards are $SE(3)$-invariant, the problem is not $SE(3)$-equivariant (Definition \ref{eq:G-equivariant_problem}), and neither is the optimal policy.

\noindent\textbf{Task}:
The task is to learn a distributed, collision-free control policy that guides the swarm to a desired formation $x_i^d,\forall i \in I_N$ via processing proprioceptive states and observations, i.e. learn  $\pi_\theta(u_i(t)|s_i(t),o_i(t))$ mapping state/observations to Gaussian distribution parametrized continuous actions $u_i(t)$. For enhanced generalization, a pool of geometric formations (circle, grid, sphere, cylinder, cube or swarming point) are used to construct diverse scenarios: 
\begin{inparaenum}
    \item \textit{Static}: a geometric formation or point is uniformly sampled and randomly placed it in the room
    \item \textit{Dynamic}: target positions and/or geometric formations or shared target point are periodically regenerated and/or formation size shrinks/expands. 
    \item \textit{Swap goals}: for a sampled geometric formation target positions are periodically randomly reassigned
    \item \textit{Swarm-vs-swarm}: swarm is split into subgroups with different formations that are periodically resampled and target positions swapped between the groups, leading to groups flying through one another 
    \item \textit{Evasion-Pursuit}: swarm tracks a moving target position, parametrized by a fast Lissajoux trajectory of random orientation/position or composite Bezier curves constructed from random points.
\end{inparaenum}

\noindent\textbf{Rewards}:  In each training episode, every quadrotor attempts to reach a designated target position of the formation while avoiding collisions with the room and other quadrotors. The reward function for every quadrotor is $\Bar{R}(s_i(t),o_i(t),u_i(t)) = \Bar{R}^x +\Bar{R}^c + \Bar{R}^s$, where $\Bar{R}^x = -c_1 ||x_i(t)-x_i^d(t)||$ a penalty motivating the quadrotor to approach the target, $\Bar{R}^c=-c_2 \mathbf{1}(||x_i(t)-x_j(t)||_2<d_{m}\,\forall j\in \mathcal{N}_i \wedge x_i(t) \notin \mathcal{X}_{room}) -c_3 \sum_{j\in \mathcal{N}_i}\max(1-||x_i(t)-x_j(t)||_2/d_p,0)$ a collision penalty and $\Bar{R}^s = - c_4 ||\omega_i(t)||_2 - c_5 ||u_i(t)||_2$ an auxiliary reward facilitating learning relatively stable controllers at the early stages of training.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.20.05 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.21.04 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.21.24 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.22.35 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.23.26 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.23.45 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.24.49 PM.png}
%   \includegraphics[width=0.245\textwidth]{files/figures/Screenshot 2024-11-15 at 6.26.13 PM.png}
%   \caption{Instances of the swarm in various scenarios}
% \end{figure}
\subsection{Architecture and Training}
To train the distributed policy we use a high-throughput, asynchronous adaptation of the Proximal Policy Optimization algorithm from \cite{petrenko2020sf} that updates the parameters of the policy to maximize the expected discounted rewards $\mathbb{E}_{\pi_\theta}[\sum_{\tau\in [0,\dots,T]} \gamma^{\tau - t} \sum_{i\in I_N} \Bar{R}(s_i(t),o_i(t),u_i(t))]$. 
As the rewards function is invariant to actions from the $SE(3)$ Lie Group, as well as the $S_N$ permutation group but the dynamics of the system are not $SE(3)$ equivariant, we leverage the structure introduced in Section \ref{section:ArtificialEquivariance} to embed these artificial symmetries in the policy parametrization, i.e. $\pi_\theta(u_i(t)|s_i(t),o_i(t)) = h_{\theta_p}(u_i(t)|\hat{\pi}_{\theta_e}(s_i(t),o_i(t)))$ where $h_{\theta_p}$ is parametrized by a simple MLP that produces the parameters for the Gaussian distribution from which the control actions are sampled and afterwards clipped, and $\hat{\pi}_{\theta_e}$ is an $SE(3)$-equivariant function. 
As the APPO training algorithm is distributed, every agent must process the information locally without multi-round communications. This is in accordance with the fact that multi-step propagation of information over a network for real-time control of high frequency systems like quadrotors is infeasible. Thus, a local view of the global graph $\mathcal{G}_t$ is used, denoted $\mathcal{G}_{i,t}$ with $|\mathcal{G}_{i,t}|=|\mathcal{N}_i|+1$, and, as each agent is unaware of the connectivity between its neighbors, a fully connected graph is constructed locally by each agent to approximate $\mathcal{G}_{i,t}$. This amounts to the assumption that $\forall (j,q)\in \mathcal{N}_i, j\neq q \neq i$ it stands that $j\in \mathcal{N}_q,q\in \mathcal{N}_j$. At every timestep $t$ of the rollout of an episode, each agent, represented by a group element $g_i(t)=(x_i(t),\mathbf{R}_i(t))\in SE(3)\,,\forall i\in I_N$, receives an neighborhood observation $o_i(t)$ on the global frame and constructs the local graph representation of the problem $\mathcal{G}_{i,t}=(\mathcal{V}_{i,t},\mathcal{H}_{i,t}), \mathcal{V}_{i,t}=\{(g_j(t),s_j(t))\,\forall j \in \mathcal{N}_i \cup \{i\}\}, \mathcal{H}_{i,t} = \{(j,k)\, \forall j,k\in \mathcal{N}_i\}$, which is used as an input to the Equivariant Graphormer of Section \ref{section:LieGraphormer}. If the observation space comprises of partial states of the neighbors that do not include elements of the group G, a local symmetry preservation is possible with node attributes $\mathcal{V}_{i,t}=\{(g_i(t),s_j(t))\,\forall j \in \mathcal{N}_i \cup \{i\}\}$ the Equivariant Graphormer is simplified according to Lemma \ref{lem:canonic} to a graphormer with input features transformed via the action induced by $g_i^{-1}$ and output features via the action of $g_i$. If the neighborhood $\mathcal{N}_i$ is constructed via a Euclidean relative distance, for the $SE(3)$ group assumption \ref{assumption:graph_invariance} stands.  The Equivariant Graphormer is an edge-preserving isomoprphism that updates the features of the nodes $\{f_j'\,\forall j \in \mathcal{N}_i \cup \{i\}\} = \mathcal{E}_{\mathcal{H}_{i,t}}(\mathcal{V}_{i,t})$ which are used to construct an equivariant mean-embedding of the neighborhood $\mu = \oplus_k \frac{1}{|\mathcal{N}_i|+1}\sum_{j\in \mathcal{N}_i\cup \{i\}} \rho_{g_i^{-1}}f_{j,k}'$.  For clarity we write $\mu = \mathcal{E}_{\theta_\epsilon}(s_i(t),o_i(t))$ to denote the aforementioned processes. The policy is, therefore, parametrized as $\pi_{\theta_p,\theta_m,\theta_\epsilon}(u_i(t)|s_i(t),o_i(t)) = h_{\theta_p}(u_i(t)| \rho_{g_i}\zeta_{\theta_m}(\mathcal{E}_{\theta_\epsilon}(s_i(t),o_i(t)),\rho_{g_i^{-1}}s_i(t)) )$ with $\zeta_{\theta_m}$ a simple MLP. A schematic of our architecture is depicted in Figure \ref{figure:schematic}.

% \begin{wrapfigure}{r}{0.3\textwidth}
%   \begin{center}
%   \includegraphics[width=1.2\textwidth, angle=-90]{files/figures/schematic.png}
%   \end{center}
%   \caption{Architecture.} \label{figure:schematic}
% \end{wrapfigure}
\begin{figure}[t]
    \centerfloat
    \includegraphics[width=1.25\textwidth, angle=0]{files/figures/schematic.png}
    \caption{Architecture schematic.} \label{figure:schematic}
\end{figure}
% \vspace{-1mm}
To further demonstrate the power of embedding symmetries in the policy and the versatility of our framework, we offer an adaptation of K-Attention from \cite{batra21corl} with $SE(3)$ symmetries. Following Lemma \ref{lem:canonic}, we can reform any architecture to an equivariant one by canonicalizing the input with the group element $g_i$ and applying the inverse group action on a hidden layer, i.e. $\pi_\theta(u_i(t)|s_i(t),o_i(t)) = h_{\theta_p}(u_i(t)|\rho_{g_i}h_{\theta_e}(\rho_{g_i^{-1}}s_i(t),\rho_{g_i^{-1}}o_i(t)))$. Other symmetry groups supported by the state's manifold can be utilized. If the manifold or part of it forms a torsor shared by various groups and the reward function is invariant to actions induced by them, the problem admits multiple symmetries. The selection process of the group if multiple choices are valid is outside the scope of this paper and is left as future work.
 
To evaluate the effect of embedding extrinsic symmetries in the learned policy, use as baselines K-Attention and DeepSets from \cite{batra21corl}, rMAPPO from \cite{yu2022the} and InfoMARL from \cite{10.5555/3618408.3619482}. With the exception of InfoMARL that utilizes GNNs, the baselines require a fixed input size, thus we fix the number of neighbors to 7 quadrotors that has been shown to be sufficient for this task in \cite{batra21corl}. The policies are trained for a total of $2\times 10^9$ steps on a single 62-core server with one A100 GPU for a swarm of 8 drones in an episodic setting, with each episode lasting 15 seconds. For the tensorial messages of the $SE(3)$-Graphormer we only use tensors of type 0 and 1. Further details regarding hyperparameters of the model, the reward function and the training algorithm are offered in Appendix \ref{appendix:hyperparams}.
Table \ref{table:results_8} summarizes the evaluation of the policies trained in all scenarios with a swarm comprising of 8 quadrotors. The evaluation metrics were averaged over 50 episodes per task and include the average collected reward per agent, the average distance to the target per agent, the average number of collisions between agents and the room per episode, the success rate (drones remaining within a small distance of their assigned target while avoiding collisions) and the inter-agent collision rate (probability of at least one collision with neighbor per agent). The policies with embedded $SE(3)$ symmetry outperform the baselines without symmetries across almost all scenarios, notably the $SE(3)$-equivariant embedding version of \cite{batra21corl}, attaining increased rewards and leading to far fewer collisions and increased success probability. The average collision rate of the $SE(3)$-Graphormer across tasks is $2.5\%$ and $4.2\%$ for $SE(3)$-K-Attention compared to $7.4\%$ for DeepSets, $11.1\%$ for InfoMARL, $16.8\%$ for K-Attention, $16.1\%$ for rMAPPO. DeepSets and InfoMARL are more aggresive, occasionally achieving better positional rewards, as observed by the average distance to target, at the expense of collision related rewards. The reduced collisions of the symmetry-enhanced policies can be explained by the fact that during training the collision instances are significantly fewer that instances without them where policies mainly optimize the position reward, meaning that even thought there are enough samples for the policy to learn target tracking, the same is not true for collision avoidance. The symmetry-enhanced policies exploit the structure of the collision avoidance specification to shrink the hypothesis class and, thus, effectively restricting the models that fit the fewer data, leading to sampling efficient and accurate learning of collision avoidance without loss of expressivity of the final policy. Overall, the $SE(3)$-enhanced policies successfully manage to guide the quadrotors to the targets with few collisions as indicated by the increased success rate.



\begin{table}[t!]
  \centerfloat
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c}
     \textsc{Scenarios}\\

\begin{tabular}{c|ccccc|ccccc|ccccc|} 
    \cline{2-16}
    & \multicolumn{5}{|c|}{\textbf{Static same goal}} & \multicolumn{5}{c|}{\textbf{Dynamic same goal}} & \multicolumn{5}{c|}{\textbf{Evasion Pursuit (Lissajous)}} \\
    \cline{2-16}
    & Rew & Dist & Col & Suc \% & IColR & Rew & Dist & Col & Suc \% & IColR & Rew & Dist & Col & Suc \% & IColR \\
    \hline\hline
    K-Attention   & -6.49 & 0.56 & 1.25 & 71.9 & 0.14 
                    &  -7.28 & 0.77 & 1.5 & 65.6 & 0.17 
                    & -8.11 & 1.25 & 1.88 & 63.5 & 0.203\\
    rMAPPO        & -7.86 & 0.70 & 2.13 & 51.6 & 0.21 
                    & -8.54 & 1.49 & 1.75 & 53.1 & 0.205
                    & -8.65 & 1.59 & 1 & 71.9 & 0.125\\
    InfoMARL      & -2.73 & 0.42 & 0.05 & 98.8 & 0.013
                    &  -4.38 & 0.65 & 0.5 & 89.4 & 0.106 
                    & -5.68 & 0.83 & 0.68 & 85.1 & 0.148\\
    K-DeepSets      & -3.24 & 0.44 & 0.1 & 96.9 & 0.006  
                    &  -4.43 & 0.69 & 0.187 & 96.1 & 0.039  
                    & -5.05 & \textbf{0.69} & 0.51 & 88.1 & 0.117\\
    % SE(2)-K-Attention (Ours) &    &   &  &   &  
    %                             &   &   &  &   &  
    %                             &  &  &   &   & \\
    SE(3)-K-Attention (Ours)  & -2.44 & 0.33 & \textbf{0} & \textbf{100} & \textbf{0} &
                        \textbf{-3.91 }& 0.87 & \textbf{0} & \textbf{100} & \textbf{0}
                        & -4.87 & 0.86 & \textbf{0.13} & 95.3 &\textbf{0.031}\\
    SE(3)-Graphormer (Ours) &  \textbf{-2.41} & \textbf{0.32} & \textbf{0} & \textbf{100} &                 \textbf{0} 
                        &-4.21 & \textbf{0.64} & 0.125 & 96.8 & 0.031 
                        & \textbf{-4.53} & 0.74 & \textbf{0.13} & \textbf{96.8} & \textbf{0.031}\\
    \hline

    & \multicolumn{5}{|c|}{\textbf{Static different goals}} & \multicolumn{5}{c|}{\textbf{Dynamic different goals}} & \multicolumn{5}{c|}{\textbf{Evasion Pursuit (Bezier)}} \\
    \cline{2-16}
    & Rew & Dist & Col & Suc \% & IColR & Rew & Dist & Col & Suc \% & IColR & Rew & Dist & Col & Suc \% & IColR \\
    \hline
    % \hline
        % \cline{1-11}
    K-Attention  & -3.88 & 0.41 & 0.5 & 87.5 & 0.063 &  
                    -5.37 & 0.74 & 0.92 & 80.2 & 0.099 
                    & -11.52 & 1.35 & 3 & 31.2 & 0.335\\
    rMAPPO      & -3.92 & 0.55 & 0.33 & 80.2 & 0.04 &  
                    -6.33 & 1.01 & 1.17 & 74.4 & 0.119 
                    &-11.8 & 2.23 & 1.08 & 45.8 & 0.225 \\
    InfoMARL    & -2.29 & \textbf{0.18} & 0.25 & 94.3 & 0.057 &
                    -3.97 & \textbf{0.60} & 0.42 & 90.5 & 0.104 
                    & -6.73 & 1.18 & 0.84 & 78.9 & 0.183\\
    K-DeepSets    & -2.73 & 0.32 & 0.07 & 98.1 & 0.017 & 
                    -4.43 & 0.72 & 0.38 & 90.9 & 0.091 
                    & -6.14 & 1.03 & 0.625 & 86.7 & 0.129\\
    % SE(2)-K-Attention (Ours) &  -2.28  & 0.31 & 0.083 & 97.9  &  0.021
    %                             &   &   &  &   &  
    %                             &  &  &   &   & \\
    SE(3)-K-Attention (Ours)   &  -1.91 & 0.24 & 0.03 & 99.2 & 0.007 
                                & -3.88 & 0.82 & 0.23 & 94.6 & 0.054 
                                & -6.71 & 1.46 & 0.37 & 80.2 & 0.082\\
    SE(3)-Graphormer (Ours)   & \textbf{-1.87} & 0.21 & \textbf{0.02} & \textbf{99.3} &                                                 \textbf{0.003}&                                                                 \textbf{-3.18} & 0.81 & \textbf{0} & \textbf{100}                                              &\textbf{0}
                             & \textbf{-5.63} & \textbf{0.97} & \textbf{0.125} & \textbf{89.0} & \textbf{0.031}\\

    \hline
    % \cline{2-16}
    & \multicolumn{5}{|c|}{\textbf{Swarm vs swarm}} & \multicolumn{5}{c|}{\textbf{Swap goals}} \\
    \cline{2-11}
    & Rew & Dist & Col & Suc \% & IColR &Rew & Dist & Col & Suc \% & IColR \\
    % \hline\hline
    \cline{1-11}\cline{1-11}
    K-Attention  & -5.16 & 0.83 & 1 & 78.1 & 0.218 & 
                    -3.91 & 0.57 & 0.50 & 88.6 & 0.113 \\
    rMAPPO      & -8.13 & 0.71 & 2 & 46.8 & 0.235 &
                    -4.01& 0.81 & 0.5 & 81.2 & 0.126 \\
    InfoMARL   & -4.15 & \textbf{0.50} & 0.71 & 83.3 & 0.167 &  
                    -3.09 & 0.41 & 0.47 & 88.7 & 0.113 \\
    K-DeepSets   &  -4.18 & 0.60 & 0.46 & 89.2 & 0.107 & 
                -3.46 & 0.42 & 0.375 & 91.4 & 0.086 \\
    % SE(2)-K-Attention (Ours) & -4.38  & 0.79  & 0.75 & 83.3  & 0.167
    %                         & -3.27 & 0.45 & 0.36 & 91.5  &  0.085\\
    SE(3)-K-Attention (Ours) &  -3.99 & 0.53 & 0.55 & 87.7 & 0.123
                                &  \textbf{-2.71} & \textbf{0.40} & 0.15 & 96.2 & 0.038 \\
    SE(3)-Graphormer (Ours) &  \textbf{-3.47} & 0.52 & \textbf{0.33} & \textbf{92.7} & \textbf{0.073} &                                                         -2.82 & 0.55 & \textbf{0.125} & \textbf{96.9} & \textbf{0.031} \\
    \cline{1-11}
\end{tabular}

\end{tabular}
  \end{adjustbox}
\caption{Evaluation for a swarm of 8 quadrotors in various scenarios.}
\label{table:results_8}
\end{table}






\subsection{Scalability Ablation Studies}
We examine the impact of embedding symmetries on the scalability of the policy when used to control swarms of increasing size with zero-shot learning. The policies of the previous section, trained for swarms of 8 quadrotors, are evaluated without further training in swarms of 16, 32, 64 and 128 quadrotors, with the metrics averaged over 50 episodes of static and dynamic scenarios (Table \ref{table:results_scalability}). As the room size remains unchanged, larger swarms lead to cluttered space, significantly increasing collisions affecting multiple drones in a cascade effect. However, the embedded symmetries are not affected by the size of the swarm leveraged locally. The symmetry-enhanced policies exhibit significantly fewer collisions than the baselines (for 128 drones the $SE(3)$-enhanced policies' collision rate rises to $\simeq16\%$ compared to $35-40\%$ for the baselines) as the swarm size progressively increases, while approaching reasonably the designated targets ($97\%$ and $84.64\%$ success rate in swarms of 64,128 compared to $<91\%$ and $<65\%$ for the baselines).

\begin{table}[t!]
  \centerfloat
\begin{adjustbox}{width=1.1\textwidth}
\begin{tabular}{c}
     \textsc{Swarm size}\\

\begin{tabular}{c|cccc|cccc|cccc|cccc|} 
    \cline{2-17}
    &  & \textbf{16} & & & & \textbf{32} & & &  & \textbf{64} & & & & \textbf{128} & & \\
    \cline{2-17}
    & Rew & Col & Suc \% & IColR & Rew & Col & Suc \% & IColR & Rew & Col & Suc \% & IColR & Rew & Col & Suc \% & IColR \\
    \hline\hline
    K-Attention   &  -5.38 & 1.6 & 84.6 & 0.154 &  
                        -5.40 &  2.8 & 86.6 & 0.134
                        & -5.58 &  7.6 & 82.8 & 0.172 
                        &  -7.70 &  69.2 & 58.9 & 0.406 \\
    rMAPPO &  -6.08 & 1.083 & 79.2 & 0.119 &
                -6.80 &  1.83 & 81.8 & 0.104 &  
                -7.79 & 16 & 57.2  & 0.352 &  
                -11.88 &  58.167 & 48.4 & 0.457 \\
    InfoMARL &  -4.07 &  0.343 & 96.7 & 0.033 & 
                    -4.72 & 2.333 & 88.02 & 0.119 & 
                    -5.19 & 11.25 & 77.3 & 0.227 &  
                    -7.03 &  40.29 & 64.6 & 0.351 \\
    K-DeepSets &  -\textbf{3.38}  & 0.2 & 97.5 & 0.025 & 
                    -3.92 & 1.875 & 90.2 & 0.098 & 
                    -4.56 & 3.8 & 90.2 & 0.121 & 
                    -10.51 &  163.17 & 64.9 & 0.348 \\
    SE(3)K-Attention (Ours)   &  -4.09 &  \textbf{0.067} & \textbf{99.2} & 0.008 & 
                                -4.41 & 0.583 & 96.6 & 0.034 & 
                                -4.96 & 2.43 & 93.7 & 0.063 &  
                                -5.66 & \textbf{12.75} &  83.77 & 0.16 \\
    SE(3)-Graphormer (Ours) &  -3.45 &  0.133 & 98.8 & \textbf{0.0125} & 
                                    \textbf{-3.69}  & \textbf{0.375} & \textbf{98.7} & \textbf{0.023}& \textbf{-4.29} & \textbf{0.82} & \textbf{97.5}  & \textbf{0.025} & 
                                    \textbf{-5.47} &  14.86 & \textbf{84.64} & \textbf{0.154}\\
    \hline
    
\end{tabular}

\end{tabular}
  \end{adjustbox}
\caption{Evaluation of zero-shot transferability to growing swarms. }
\label{table:results_scalability}
\end{table}

















% \begin{table}[H]
%   \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{c}
%      \textbf{Scenarios}\\

% \begin{tabular}{c|ccccc|ccccc|} 
%     \cline{2-11}
%     & \multicolumn{5}{|c|}{\textbf{Static same goal}} & \multicolumn{5}{c|}{\textbf{Dynamic same goal}} \\
%     \cline{2-11}
%     & Reward & Distance & Collisions & Success \% & Collision rate & Reward & Distance & Collisions & Success \% & Collision rate \\
%     \hline\hline
%     K-Attention   & -7.297 & 0.616 & 2.25 & 52.1 & 0.479 &  -9.519 & 0.981 & 3.083 & 50 & 0.5 \\
%     rMAPPO        & -7.695 & 0.707 & 1.5 & 59.4 & 0.312 & -10.271 & 1.038 & 1.917 & 59.4 & 0.385 \\
%     InfoMARL      & -5.341 & 0.428 & 0.25 & 93.8 & 0.063 &  -7.711 & 0.802 & 0.8 & 84.4 & 0.156 \\
%     DeepSets      & \textbf{-4.197} & \textbf{0.285} & 0.05 & 98.8 & 0.012  &  -7.054 & 0.757 & 0.45 &                      89.4 & 0.106  \\
%     SE(3)-K-Attention (Ours)  & -4.689 & 0.323 & 0.079 & 98.1 & 0.019 &   -7.147 & 0.796 & \textbf{0.167} &                                \textbf{95.8} &\textbf{ 0.041} \\
%     SE(3)-Graphormer (Ours) &  -4.554 & 0.330 & \textbf{0} & \textbf{100} & \textbf{0}  & -\textbf{6.674} &                           \textbf{0.756} & 0.25 & 93.8 & 0.063 \\
%     \hline

%     & \multicolumn{5}{|c|}{\textbf{Static different goals}} & \multicolumn{5}{c|}{\textbf{Dynamic different goals}} \\
%     \cline{2-11}
%     & Reward & Distance & Collisions & Success \% & Collision rate & Reward & Distance & Collisions & Success \% & Collision rate \\
%     \hline\hline
%     K-Attention  & -5.856 & 0.417 & 0.56 & 89.4 & 0.106 &  -8.293 & 0.836 & 0.688 & 84.4 & 0.157 \\
%     rMAPPO & -6.624 & 0.571 & 0.55 & 76.9 & 0.125 &  -9.883 & 1.203 & 1.25 & 69.3 & 0.276 \\
%     InfoMARL   &\ -3.837 & 0.171 & 0.12 & 98.1 & 0.019 &  -6.831 & 0.745 & 0.4 & 91.25 & 0.088 \\
%     DeepSets   & \textbf{-3.312} & \textbf{0.139} & 0.1 & 97.5 & 0.025 & \textbf{-5.782} & \textbf{0.542}               & 0.75 & 82.81 & 0.172 \\
%     SE(3)-K-Attention (Ours)   &  -4.016 & 0.226 & \textbf{0} & \textbf{100} & \textbf{0} & -6.955 &                    0.825 & 0.125 & 96.9 & 0.031 \\
%     SE(3)-Graphormer (Ours)   & -3.784 & 0.197 & \textbf{0} & \textbf{100} & \textbf{0} &  -6.239 & 0.793       & \textbf{0.05} & \textbf{98.8} & \textbf{0.013} \\

%     \hline
%     & \multicolumn{5}{|c|}{\textbf{Swarm vs swarm}} & \multicolumn{5}{c|}{\textbf{Swap goals}} \\
%     \cline{2-11}
%     & Reward & Distance & Collisions & Success \% & Collision rate & Reward & Distance & Collisions & Success \% & Collision rate \\
%     \hline\hline
%     K-Attention  & -7.706 & 0.744 & 0.972 & 80.2 & 0.198 & -6.678 & 0.571 & 0.417 & 90.6 & 0.094 \\
%     rMAPPO     & -8.173 & 0.877 & 1.25 & 68.8 & 0.281 &  -7.633& 0.776 & 0.875 & 77.3 & 0.203 \\
%     InfoMARL   & -6.105 & 0.505 & 0.417 & 90.6 & 0.093 &  -5.291 & 0.447 & 0.9 & 81.2 & 0.188 \\
%     DeepSets   &  \textbf{-5.56} & \textbf{0.471} & 0.6 & 85 & 0.15 & \textbf{-4.524} & \textbf{0.307} &                       0.667 & 85.2 & 0.148 \\
%     SE(3)-K-Attention (Ours) &  -6.605 & 0.597 & 0.543 & 87.5 & 0.125 &  -5.225 & 0.407 & 0.279 & 93.5 &                        0.065 \\
%     SE(3)-Graphormer (Ours) &  -6.04 & 0.596 & \textbf{0.333} & \textbf{91.7} & \textbf{0.083} & -5.124 &               0.425 & \textbf{0} & \textbf{100} & \textbf{0} \\

%     \hline
%     & \multicolumn{5}{|c|}{\textbf{Evasion-Pursuit (Lissajous+Bezier)}} & \multicolumn{5}{c}{}\\
%     \cline{2-6}
%     & Reward & Distance & Collisions & Success \% & Collision rate & \multicolumn{5}{c}{}\\
%     \cline{1-6}
%     K-Attention  & -10.964 & 1.085 & 1.9 & 62.5 & 0.369 &&&&\\
%     rMAPPO     & -14.224 & 1.389 & 2.25 & 50.6 & 0.438 &&&&\\
%     InfoMARL   & -9.446 & 0.899 & 0.65 & 86.9 & 0.131 &&&&\\
%     DeepSets   & -8.835 & 0.941 & \textbf{0} & \textbf{98.9} & \textbf{0} &&&&\\
%     SE(3)-K-Attention (Ours)   & -9.986 & 0.993 & 0.714 & 87.5 & 0.121 &&&&\\
%      SE(3)-Graphormer (Ours)   & \textbf{-8.801} & \textbf{0.899 }& 0.25 & 93.8 & 0.062 &&&&\\

%      \cline{1-6}
% \end{tabular}

% \end{tabular}
%   \end{adjustbox}
% \caption{Evaluation for a swarm of 8 quadrotors in various scenarios.}
% \label{table:results_8}
% \end{table}



% \begin{tabular}{c|ccccc|ccccc|} 
%     \cline{2-11}
%     &  & & \textbf{16} & & & & & \textbf{32} & & \\
%     \cline{2-11}
%     & Reward & Distance & Collisions & Success \% & Collision rate & Reward & Distance & Collisions & Success \% & Collision rate \\
%     \hline\hline
%     K-Attention   &  -5.783 & 0.391 & 1.6 & 84.6 & 0.154 &  -5.405 & 0.324 & 2.8 & 86.6 & 0.134 \\
%     rMAPPO &  -6.08 & 0.509 & 1.083 & 79.2 & 0.119 & -6.801 & 0.533 & 1.83 & 81.8 & 0.104 \\
%     InfoMARL &  -4.073 & 0.198 & 0.343 & 96.7 & 0.033 & -4.728 & 0.207 & 2.333 & 88.02 & 0.119 \\
%     DeepSets &  -\textbf{3.379} & \textbf{0.126} & 0.2 & 97.5 & 0.025 & \textbf{-3.691} & \textbf{0.103}                    & 1.875 & 90.2 & 0.098 \\
%     SE(3)K-Attention (Ours)   &  -4.091 & 0.229 & \textbf{0.067} & \textbf{99.2} & 0.008 & -4.411 & 0.238                   & 0.583 & 96.6 & 0.034 \\
%     SE(3)-Graphormer (Ours) &  -3.854 & 0.207 & 0.133 & 98.8 & \textbf{0.0125} & -3.908 & 0.171 &                           \textbf{0.375} & \textbf{98.7} & \textbf{0.023}\\
%     \cline{2-11}
%     &  & & \textbf{64} & & & & & \textbf{128} & & \\
%     \cline{2-11}
%     & Reward & Distance & Collisions & Success \% & Collision rate & Reward & Distance & Collisions & Success \% & Collision rate \\
%     \hline\hline
%     K-Attention  & -5.588 & 0.271 & 7.6 & 82.8 & 0.172 &  -7.706 & 0.552 & 69.2 & 58.9 & 0.406 \\
%     rMAPPO     &  -7.799 & 0.641 & 16 & 57.2  & 0.352 &  -11.883 & 1.148 & 58.167 & 48.4 & 0.457 \\
%     InfoMARL   & -5.198 & 0.174 & 11.25 & 77.3 & 0.227 &  -7.029 & 0.436 & 40.29 & 64.6 & 0.351 \\
%     DeepSets   & -4.562 & \textbf{0.095} & 3.8 & 90.2 & 0.121 & -10.503 & 0.623 & 163.17 & 64.9 & 0.348 \\
%     SE(3)-K-Attention (Ours) & -4.963 & 0.274 & 2.43 & 93.7 & 0.063 &  -5.668 & 0.288 & \textbf{12.75} & 
%                           83.77 & 0.16 \\
%     SE(3)-Graphormer (Ours)   & \textbf{-4.293} & 0.185 & \textbf{0.82} & \textbf{97.5}  & \textbf{0.025}                   & \textbf{-5.472} & \textbf{0.266} & 14.86 & \textbf{84.64} & \textbf{0.154}\\
%     \hline
    
% \end{tabular}

% \end{tabular}
%   \end{adjustbox}
% \caption{Evaluation of zero-shot transferability to growing swarms. }
% \label{table:results_scalability}
% \end{table}

==> Extended_version_files/Introduction_extended.tex <==

\section{Introduction}

The study of dynamical systems in multi-agent settings, such as robotic swarms, has garnered significant attention due to its wide-ranging applications in areas like autonomous navigation, environmental monitoring, target tracking, collaborative manipulation, localization and mapping, power grid management etc. Since dataset of expert demonstrations for large-scale systems are rare, multi-agent reinforcement learning (MARL) has emerged as a powerful framework for enabling agents to learn complex, coordinated behaviors from interactions with their environments. However, the inherently high-dimensional and decentralized nature of multi-agent systems poses significant challenges, particularly in terms of scalability, generalization, and data efficiency for any deep learning approach. To enhance generalization, synthetic samples can be generated by applying symmetry transformations to the original data, increasing diversity without additional sampling (e.g. \cite{NEURIPS2020_e615c82a}). Data augmentation, though, increases computation time and offers no generalization assurances. Outside of data augmentation, one promising avenue to address these challenges lies in leveraging the symmetries of dynamical systems as an inductive bias in the network construction to shrink the hypothesis class of the learned controller and, thus, effectively restrict the models that fit it. This leads to efficient and accurate learning of distributed controllers without expressivity loss. Equivariant and geometric deep learning have shown promising results in shape reconstruction \cite{chatzipantazis2023mathrmseequivariant}, pedestrian and skeleton motion prediction \cite{Xu2023EqMotionEM}, atomic and molecular dynamics \cite{Batzner2021E3equivariantGN}, robot planning \cite{zhao2024mathrm,wang2024equivariant} and computer vision \cite{weiler2018learning}. 

From an RL perspective, the existence of symmetries morphs into equivalence of state-action pairs under a group transformation. Consider the example of robotic arm whose goal is to move an object to a target position, and rotating the entire setup (object, target, and arm) by $90^{\circ}$ leaves the task unchanged. This implies that the original state-action pair $(x,u)$ and the rotated state-action pair $(T_g(x),L_g(u))$ are equivalent in terms of outcomes, thus the policy $\pi(u|x)$ only needs to learn one mapping for each equivalence class, rather than separately learning the same behavior for all symmetrically related pairs. The presence of symmetries allows RL algorithms to exploit these equivalences by directly reducing the hypothesis space and improves sample efficiency (fewer unique samples are needed to learn the policy) and generalization (the policy learned for one pair generalizes to all equivalent pairs). This observation means that symmetry-aware methods effectively operate on a reduced state-action space, corresponding to the equivalence classes rather than individual pairs. This enabled \cite{Yu2022EquivariantRL} to construct an $S^1$ symmetry out of the quadrotor's state, reducing the input features of the policy to elements of the equivalence class. 

Though working with a reduced state-action space benefits for off-the-self neural architectures to parametrize the policy, it may restrict the expressivity of the policy, thus motivating the design of neural architectures that inherently respect the symmetries as an inductive bias via sharing parameters across symmetric components. Omnipresent in homogeneous multi-agent systems is permutation equivariance, i.e. all robot dynamics and reward functions are identical, so indexing is interchangeable. This discrete $S_n$ symmetry, leading to wight sharing amongst agents, is the basis of the representation power of Graph Nueral Networks, exhibited in \cite{jiang2020graphconvolutionalreinforcementlearning,tzes2023graph}. However, in continuous geometric symmetries weight sharing would require a discretization of equivalence classes that is memory intractable, though fast and expressive \cite{bekkers2024fast}. To that end, equivariant-by-construction policies utilize symmetry-preserving operations via, e.g. spherical harmonics \cite{fuchs2020se3transformers}. To exploit such properties in RL, \cite{NEURIPS2020_2be5f9c2} proposed a $C_n$ equivariant architecture to discrete rotations and \cite{pmlr-v164-wang22j,wang2020policylearningse3action} extended it to continuous $SO(2)$ and $SE(2)$ symmetries. 
The generalization capacity of equivariant policy learning for a single agent has been demonstrated in symmetric locomotion (\cite{su2024leveraging}), planning \cite{zhao2023integrating}, grasping and manipulation (\cite{pmlr-v164-wang22j,nguyen2023equivariant}). 






If a swarm of drones is tasked with maintaining a formation, rotating the entire formation or relabeling the drones doesn't change the task, so any state-action pair after rotation or relabeling is equivalent to the original. A symmetry-aware RL algorithm learns a single policy for the equivalence class, enabling generalization to unseen formations or configurations.

% However, in multi-robot systems identifying these symmetries is more involved as robot-interaction occasionally breaks existing ones. If certain agents are assigned leader roles in specific tasks, treating all agents as symmetric may lead to suboptimal policies. Environmental factors like obstacles or communication delays may create asymmetries that the symmetry-aware policy cannot handle effectively.



This paper focuses on symmetry exploitation in cooperative-competitive MARL problems. 

\subsection{Contributions}
All the works in the aforementioned literature review attempt to utilize symmetries as inductive biases in policy learning, which, however, presumes that the system exhibits said symmetries. In practice, most dynamical systems exhibit little to no symmetries. To the best of our knowledge, this is the first paper that attempts to construct a framework on how to leverage symmetries in policies, even if the system is not endowed with them. Our contributions are outlined below:
\begin{itemize}
\item A formalization of the symmetry properties of multi-robot dynamical systems and the conditions under which optimal policies are equivariant functions to be approximated by equivariant networks. These conditions showcase the restrictive nature of current equivariant RL methods to systems with explicit symmetries shared by the task specification.

\item A methodology for embedding artificial arbitrary symmetries in systems where intrinsic symmetries are insufficient or broken, thus broadening the applicability of equivariant learning frameworks to any multi-agent dynamical system.

\item The introduction of a Group Equivariant Graphormer architecture tailored to distributed swarming tasks. This network is by design modular in terms of the symmetry considered (any group compatible with the manifold of the dynamics, discrete or continuous), in contrast to the vast majority of networks in the literature. 

\end{itemize}
By embedding artificial symmetries, our approach demonstrates enhanced learning efficiency and generalization capabilities, paving the way for broader adoption of symmetry-aware methods in multi-agent reinforcement learning and control, even when the original dynamical systems do not exhibit them. The subsequent sections outline the theoretical underpinnings of equivariant dynamics, introduce the proposed framework, and validate its efficacy through extensive experimentation on a swarm of $SE(3)$ symmetry braking quadrotors that showcases the effectiveness of our scheme regarding scalability and robustness

\subsection{Literature Review}

\noindent\textbf{Symmetries in RL \& Control}: Exploiting symmetries in MDPs has been introduced in \cite{Ravindran2001SymmetriesAM,Zinkevich2001SymmetryIM}. Recent work focus on symmetries for deep RL as a data-efficient approach via embedding symmetries in policy networks (\cite{vanderpol2020plannableapproximationsmdphomomorphisms,NEURIPS2020_2be5f9c2,zhu2022sampleefficientgrasplearning,simm2020symmetryawareactorcritic3dmolecular}), invariant data augmentation (\cite{NEURIPS2020_e615c82a,kostrikov2021imageaugmentationneedregularizing}), symmetric filters (\cite{pmlr-v37-clark15}), equivariant trajectory augmentation (\cite{pmlr-v162-weissenbacher22a,9158366,mavalankar2020goal}). \cite{NEURIPS2020_2be5f9c2} proposed an equivariant architecture on $C_n$ symmetries of discrete rotations and \cite{pmlr-v164-wang22j,wang2020policylearningse3action} extended it to continuous $SO(2)$ and $SE(2)$ symmetries. \cite{mondal2020groupequivariantdeepreinforcement} applied an $E(2)$-equivariant network to Q-learning in an Atari game domain. \cite{Yu2022EquivariantRL}  constructed an $S^1$ symmetry for a quadrotor policy. \cite{sonmez2024exploitingsymmetrydynamicsmodelbased} used Cartan’s moving frame method to construct equivalent states and invariant input features for the policy, independent of the reward function. The effectiveness of learning equivariant policies, with continuous or discrete symmetries, for a single agent has been demonstrated in symmetric locomotion (\cite{su2024leveraging,abdolhosseini2019learning,ordonez2023discrete}), planning \cite{zhao2023integrating}, grasping and manipulation (\cite{zhu2022sample,10160728,pmlr-v164-wang22j,nguyen2023equivariant}). Unlike the aforementioned that assume apriori knowledge of symmetries, \cite{pmlr-v162-weissenbacher22a} infers symmetries from data and augments the training data using these symmetries.
Symmetries have been, also, utilized in control and state estimation (\cite{1103421,MAHONY2013617,mahony2020equivariantfilterdesignkinematic,mahony2020equivariantsystemstheoryobserver}), dynamic programming \cite{maidens2018symmetryreductiondynamicprogramming} and reachability analysis \cite{8277172} to reduce computational complexity. 
However, these approaches are only suitable for single agent or centralized
multi-agent controllers for system dynamics and tasks with inherent symmetries, thus severely limiting their applicability. We solve the problem of leveraging symmetries, even in systems that do not exhibit them, while still allowing distributed execution.



\noindent\textbf{Permutation symmetries in multi-agent systems}:
Permutation invariance is another symmetry often appearing in homogeneous MARL where the dynamics and reward functions of all agents are the same, so identities are disregarded and any indexing permutation of them would lead to the same indexing permutation of the optimal actions as only the observations are used. This property directly limits the required sample complexity for training the distributed policy, and can be usually exploited via policy sharing (\cite{chen2022communicationefficient,NIPS2017_c2ba1bc5}), permutation equivariant critics (\cite{Almasan_2022,liu2019picpermutationinvariantcritic,rashid2020monotonicvaluefunctionfactorisation,liu2019picpermutationinvariantcritic}) or mean field approximation (\cite{pmlr-v80-yang18d}). For policy sharing, a common approach is to use coordination graphs to explicitly formulate symmetries and learn local Q-functions. \cite{pmlr-v119-boehmer20a} factored the joint value function according to a coordination graph into payoffs between pairs of agents while \cite{Pol2016Coordinated} considered the deconstruction of the problem as a linear combination of local subproblems. Another approach is to use graph-based networks that are inherently permutation equivariant, like \cite{jiang2020graphconvolutionalreinforcementlearning}. \cite{pmlr-v119-hu20a} used known permutation symmetries to improve zero-shot coordination in game that require coordinated symmetry breaking. Though, permutation equivariant methods exploit the homogeneity structure, they ignore the geometry of the problem. We leverage both by introducing a group equivariant graph neural network.


\noindent\textbf{Geometric Symmetries in MARL}: From a geometric standpoint, few symmetries in MARL have been explored. \cite{vanderpol2022multiagentmdphomomorphicnetworks} introduced Multi-Agent MDP Homomorphic Networks to utilize $C_n$ symmetries arising between different configurations of the agents and their local observations, with, however, the input size of the proposed network that scaling with $|C_n|$ and Euclidean equivariance only preserved for discrete rotations. \cite{pmlr-v202-chen23i} inject an $E(3)$ symmetry in subequivariant morphology-agnostic RL policies and Q-function such that the policy can generalize to all directions, improving exploration efficiency.
\cite{chen2023rm} characterize a subclass of Markov games with a general notion of symmetries that admits the existence of symmetric optimal values-policies and embed $E(3)$ constraints in graph-based multi-agent actor-critic methods. \cite{mcclellan2024boostingsampleefficiencygeneralization} used an adaptation of EGNNs to demonstrated how $O(n)$ equivariance boosts sample efficiency and generalization in MARL. All of these works use equivarinace-by-construction policies, usually based on equivariant operations on message-passing networks (\cite{pmlr-v139-satorras21a,pmlr-v139-schutt21a,bekkers2024fast}), lifting to the lie algebra (\cite{finzi2020generalizing,mironenco2024lie,macdonald2022enablingequivariancearbitrarylie}), group infinitesimal generators (\cite{NEURIPS2021_148148d6}), gauge theory (\cite{NEURIPS2021_e57c6b95,dehaan2021gaugeequivariantmeshcnns}), vectorized features (\cite{Deng2021VectorNA}) or steerability via harmonic analysis (\cite{thomas2018tensor,fuchs2020se3transformers}) This assumes knowledge of a predefined geometric symmetry of the problem and, thus, are not transferable to MARL problems with different symmetries. We propose a simple but modular Group Equivariant Graphormer that can be adapted for a variety of symmetries in differently structured MARL problems via canonicalizing group actions on tensorial graph features. Furthermore, all of these works attempt to exploit only existing symmetries in the systems, whereas the current paper extends to systems with partial or broken symmetries via embedding them in associated artificial symmetries-enhanced systems to include desirable equivariant properties.



% \st{Lagrangian dynamical systems may exhibit symmetries that one can exploit to shrink the hypothesis class of the learned controller and, thus, effectively restrict the models that fit it, leading to efficient and accurate learning without loss of expressivity. 
 
%  By encoding appropriate geometry-inspired inductive biases in the representation of the features, one may, further, attain a level of explainability of the learned model. Multi-agent dynamical systems usually exhibit time-invariant geometric group symmetries in the joint tensor bundle space of the generalized coordinates, e.g. fundamental atomic interactions may remain invariant under time-invariant geometric transformations, as they abide by the energy conservation principle, prescribed specifications of the task, dynamical models etc. Regarding the scalability of the distributed controller, as it is a learned function of local information, increased accuracy in the representations should lead to a significant increase in generalizability to graphs of growing cardinality, provided these graphs converge to the same graphon as the one the model was trained on.}




% \par\textbf{MARL}....
% \begin{itemize}
%   \item Multi-Agent Reinforcement Learning is A Sequence Modeling Problem
%   \item The Surprising Effectiveness of PPO in Cooperative Multi-Agent Games
% \end{itemize}


% \par\textbf{RL for quadrotors}....
% \begin{itemize}
%   \item Learning to Fly in Seconds
%   \item QuadSwarm: A Modular Multi-Quadrotor Simulator for Deep Reinforcement Learning with Direct Thrust Control
% \end{itemize}

% \par\textbf{Distributed Learning for Swarms}....
% \begin{itemize}
%   \item Decentralized Control of Quadrotor Swarms with End-to-end Deep Reinforcement Learning
%   \item Scalable Multi-Agent Reinforcement Learning through Intelligent Information Aggregation
%   \item 
% \end{itemize}


% \subsubsection{Equivariant Deep Learning}

% \url{https://github.com/Chen-Cai-OSU/awesome-equivariant-network?tab=readme-ov-file#application}

% \begin{itemize}
%   \item SE(3)-Transformers: 3D Roto-Translation Equivariant Attention Networks
%   \item Enabling Equivariance for Arbitrary Lie Groups
%   \item LieGG: Studying Learned Lie Group Generators
%   \item A Hitchhiker’s Guide to Geometric GNNs for 3D Atomic Systems
%   \item Automatic Symmetry Discovery with Lie Algebra Convolutional Network
%   \item EqMotion: Equivariant Multi-agent Motion Prediction with Invariant Interaction Reasoning
%   \item Generalizing Convolutional Neural Networks for Equivariance to Lie Groups on Arbitrary Continuous Data
%   \item SE(3) FRAME EQUIVARIANCE IN DYNAMICS MODELING AND REINFORCEMENT LEARNING
%   \item SE(3) Equivariant Graph Neural Networks with Complete Local Frames
%   \item Geometry-Complete Perceptron Networks for 3D Molecular Graphs
%   \item EQUIVARIANT GRAPH NEURAL OPERATOR FOR MODELING 3D DYNAMICS
%   \item FAST, EXPRESSIVE SE(n) EQUIVARIANT NETWORKS THROUGH WEIGHT-SHARING IN POSITION-ORIENTATION SPACE
%   \item Equivariant and Steerable Neural Networks
%   \item Approximately Equivariant Graph Networks
%   \item Approximately Equivariant Networks for Imperfectly Symmetric Dynamics
%   \item Tensor field networks: Rotation- and translation-equivariant neural networks for 3D point clouds
%   \item Vector Neurons: A General Framework for SO(3)-Equivariant Networks
%   \item Group Equivariant Convolutional Networks
%   \item General E(2)-Equivariant Steerable CNNs
%   \item Gauge Equivariant Transformer
%   \item Clifford-Steerable Convolutional Neural Networks
%   \item NEURAL EPDOS: SPATIALLY ADAPTIVE EQUIVARIANT PARTIAL DIFFERENTIAL OPERATOR BASED NETWORKS
%   \item On the Expressive Power of Geometric Graph Neural Networks
%   \item Equivariant Hamiltonian Flows
%   \item Equivariant Manifold Flows
%   \item Independent SE(3)-Equivariant Models for End-to-End Rigid Protein Docking
%   \item Universal Invariant and Equivariant Graph Neural Networks
% \end{itemize}



% \subsubsection{Equivariant Reinforcement Learning}....
% \begin{itemize}
%   \item Equivariant Reinforcement Learning for Quadrotor UAV
%   \item Subequivariant Graph Reinforcement Learning in 3D Environments
%   \item SO(2)-EQUIVARIANT REINFORCEMENT LEARNING
%   \item BOOSTING MULTIAGENT REINFORCEMENT LEARNING VIA PERMUTATION INVARIANT AND PERMUTATION EQUIVARIANT NETWORKS
%   \item Subequivariant Reinforcement Learning in 3D Multi-Entity Physical Environments
%   \item Cooperative Multi-Agent Fairness and Equivariant Policies
%   \item MULTI-AGENT MDP HOMOMORPHIC NETWORKS
%   \item EqR: Equivariant Representations for Data-Efficient Reinforcement Learning
%   \item E(3)-Equivariant Actor-Critic Methods for Cooperative Multi-Agent Reinforcement Learning
%   \item Symmetry-Aware Actor-Critic for 3D Molecular Design
%   \item Equivariant Q Learning in Spatial Action Spaces
% \end{itemize}
% \par\textbf{Graphs and permutation symmetries in multi agent reinforcement learning }...

% \subsubsection{Equivariance in control \& robotics}...
% \begin{itemize}
%   \item EQUIVARIANT FILTER DESIGN FOR KINEMATIC SYSTEMS ON LIE GROUPS
%   \item Tracking control on homogeneous spaces: the Equivariant Regulator (EqR)
%   \item Overcoming bias: Equivariant filter design for biased attitude estimation with online calibration
%   \item Equivariant systems theory and observer design
%   \item Equivariant Systems Theory and Observer Design for Second Order Kinematic Systems on Matrix Lie Groups
%   \item Equivariant Symmetries for Inertial Navigation Systems
%   \item An Equivariant Approach to Robust State Estimation for the ArduPilot Autopilot System
%   \item EXPLOITING EQUIVARIANCE IN THE DESIGN OF TRACKING CONTROLLERS FOR EULER-POINCARE SYSTEMS ON MATRIX LIE GROUPS
%   \item Equivariant Filter (EqF)
%   \item EXPLOITING DIFFERENT SYMMETRIES FOR TRAJECTORY TRACKING CONTROL WITH APPLICATION TO QUADROTORS
%   \item Diffusion-EDFs: Bi-equivariant Denoising Generative Modeling on SE(3) for Visual Robotic Manipulation
%   \item Sample Efficient Grasp Learning Using Equivariant Models
%   \item FOURIER TRANSPORTER: BI-EQUIVARIANT ROBOTIC MANIPULATION IN 3D
%   \item Robotic Manipulation Learning with Equivariant Descriptor Fields: Generative Modeling, Bi-equivariance, Steerability, and Locality
%   \item Multi-Robot Active Mapping via Neural Bipartite Graph Matching
%   \item The Surprising Effectiveness of Equivariant Models in Domains with Latent Symmetry
%   \item Equivariant Transporter Network
%   \item 
% \end{itemize}





==> Extended_version_files/Preliminaries_extended.tex <==
\section{Preliminaries}

\subsection{Group Theory \& Representations}
A group $(G,\cdot)$ is a set $G$ equipped with an operator $\cdot:G\times G \rightarrow G$ that satisfies:
\begin{itemize}
    \item Identity: $\exists e \in G$ such that $e \cdot g = g \cdot e = e$
    \item Associativity: $\forall g,h,f \in G,\, g\cdot (h \cdot f) = (g \cdot h) \cdot f$
    \item Inverse: $\forall g \in G,\, \exists g^{-1}$ such that $g^{-1} \cdot g = g \cdot g^{-1} = e$
\end{itemize}
Additional to its structure we can define the way that the group elements act on a space $X$ via a group action:
\begin{definition_}\label{definitioin:group_action}
A map $L_g: X\to X$ is called an action of group element $g\in G$ on $X$ if it satisfies the following properties:
\begin{itemize}
    \item if $e$ is the identity element $L_e[x]=x$ for all $x\in X$
    \item $L_g\circ L_h=L_(g\cdot h)$ for all $g,h\in G$
\end{itemize}
\end{definition_}
When $X$ is vector space, we can define the action of the group through a linear group representation. Specifically:
\begin{definition_}
A linear group representation $(V,\rho)$ of a group $G$ is a map $\rho:G\to GL(V)$ from group $G$ to the general linear group $GL(V)$. The group action is then defined by the linear operator $L_g[x]=\rho(g)x$ for all $x\in V, g\in G$.
\end{definition_}
Note here that a group action on a given space $X$ allow us to group different elements of $X$ in sets of orbits. More precisely given a group action $L_*$ an orbit of a element $x\in X$ is the set $\mathcal{O}_x^{L_*}=\left\{L_g[x]|g\in G\right\}$. 

\noindent In many application we require functions that respect the structure of of a  group acting on their domain and codomain. This means that we require an action of a group element on the input of the function to correspond to an action of the group on the output of this function. For example given a system of point masses with positions and acceleration  where we want to predict the overall momentum, we require the estimated momentum for all rotated version of the input to rotate appropriately. We refer to these functions as equivariant and we formally define them as follow:
\begin{definition_}
Given a group $G$ and corresponding group actions actions $L_g:X\to X$, $T_g:X\to X$ for $g\in G$  a function $f:X\to Y$ is said to be $(G,L_*,T_*)$ equivariant if and only if: 
\begin{equation}
    T_g\left[f(x)\right]=f\left(L_g[x]\right)\quad \forall x\in X, g\in G
\end{equation}
\end{definition_}
 
\iffalse
Note that groups are not necessarily commutative, i.e. $\exists (G,\cdot)$ such that $g \cdot h \neq h \cdot g, \forall g,h \in g$.  If the binary operation is commutative, the group is abelian. If the set $G$ is equipped with a topology with the binary operator and the inverse map continuous, $G$ is a topological group. If that topology is compact, the group $G$ is a compact group. If G is a smooth manifold and the binary operator and the inverse map are smooth, it is a Lie group. A subgroup $(H, ·)$ of a group $(G, ·)$ is a group such that $H \subseteq G$. Given a group $(G,\cdot)$, we denote the action on the space $X$ with $L_g:X \rightarrow X,\, \forall g \in G$. The transformation/operator satisfies the following properties:
\begin{inparaenum}
    \item Trivial action: for $e\in G$ with $e \cdot g = g \cdot e = e$,   $L_e[g]=g,\, \forall g \in G$
    \item Closure: $\forall g,h,q \in G$, $L_g \circ L_h [q] = L_{g\cdot h}[q]$
\end{inparaenum}
where $\circ$ is the composition of transforming actions. If $\forall x,y \in X,\, \exists g\in G$ such that $L_g[x]=y$, then $X$ is a homogeneous space for group $G$.
\begin{definition_}
    A \textbf{\textit{representation}} $(G,\rho)$ of an algebraic group is a morphism $\rho:G \rightarrow GL(V)$ mapping linearly from the group $G$ to the general linear group $GL(V)$, for $V$ some vector space over some field, with the group action defined by the linear operator, i.e. $L_g[x]=\rho(g)x\,,\, \forall x \in V, g\in G$. 
\end{definition_}
If the morphism $\rho(\cdot)$ is a group homeomorphism, i.e. $\rho(g\cdot h)= \rho(g) \cdot \rho(h)\,,\, \forall g,h \in G$, then the representation $(V,\rho)$ is a linear group representation. Moreover, for the group homeomorphisms, using the identity property it stands that $\rho(g^{-1})= \rho(g)^{-1} \forall g \in G$. The \textbf{\textit{degree}} of a linear representation is the dimension of the corresponding vector space $V$ .

\begin{definition_}[\textbf{Equivariance}] Given group $G$ and the set of actions $L_g:X \rightarrow X\,,\, \forall g\in G$ and the the set of actions $T_g:Y \rightarrow Y\,,\, \forall g\in G$, the map $f:X \rightarrow Y$ is \textbf{$(G,L_*,T_*)$-equivariant} if $T_g[f(x)]=f(L_g[x])\quad \forall x\in X, g\in G$
\end{definition_} 
\begin{definition}[\textbf{Invariance}]
Given actions $L_g:X \rightarrow X\,,\, \forall g\in G$, the map $f:X \rightarrow Y$ is \textbf{$(G,L_*,T_*)$-invariant} if $f(x)=f(L_g[x])\; \forall x\in X, g\in G$. Invariance is a form of equivariance with $T_g[f(\cdot)]=f(\cdot)$.
\end{definition} 
A unitary finite dimensional representation of a group $G$ is a representation of $G$ on a complex finite dimensional vector space $V$ over $\mathbb{C}$ equipped with a ${G}$-invariant positive definite Hermitian form (linear in the first argument, anti-linear in the second), i.e. $<\rho(g)v, \rho(g)w>=<v,w>\,,\,\forall g \in G,v,w \in V$. A \textbf{Lie group} is a smooth manifold whose underlying set of elements is equipped with the structure of a group and endowed with differentiable group operations. A real Lie group is a compact/connected Lie group if its underlying topological space is compact/connected. Every connected finite dimensional real Lie group is homeomorphic to a product of a compact Lie group, i.e. the maximal compact subgroup, and a Euclidean space.

\subsubsection{Tensors}
.......
\fi
\subsection{Notation}
    Let $\mathcal{X}$ be a smooth manifold and $T_x\mathcal{X}$ the tangent space at an arbitrary $x\in \mathcal{X}$. A smooth vector field is a smooth map $f:\mathcal{X}\rightarrow T\mathcal{X}$ with $f(x)\in T_x\mathcal{X}$. The set of smooth vector fields on a manifold $\mathcal{X}$, denoted $\mathfrak{X}(\mathcal{X})$, is a linear infinite dimensional vector space. Let $G$ be a d-dimension real Lie group, with identity element $e$. The tangent space $T_g \mathcal{X}$ for $g\in G$ is a real d-dimensional vector space and the associated Lie algebra of $G$, denoted $\mathfrak{g}:=T_eG$, is isomorphic to $\mathbb{R}^d$. For vector fields $f_1,f_2 \in \mathfrak{X}(\mathcal{X})$ the Lie-bracket $[f_1,f_2]\in \mathfrak{X}(\mathcal{X})$ is anti-symmetric and respects the Jacobi equation, while $\mathfrak{X}(\mathcal{X})$ is a Lie algebra. For $g \in G$, the adjoint map $Ad:G\times \mathfrak{g} \rightarrow \mathfrak{g}$ amounts to a change of basis on the Lie algebra, i.e. $Ad_g(q)=dL_g (dR_g (q))$ for $q\in \mathfrak{g}$ and $dL_g q,dR_g q \in T_gG$ the left and right group translation induced on the algebra respectively. For matrix Lie groups, $dL_g q= g\cdot q,\,dR_gq=q\cdot g$ and $Ad_gq=g\cdot q \cdot g^{-1}$. For a smooth manifold $\mathcal{X}$ and Lie group $G$, the left natural action $\phi:G \times \mathcal{X} \rightarrow \mathcal{X}$ satisfies $\phi(e,x) = x,\forall x\in \mathcal{X}$ and $\phi(\hat{g},\phi(g,x))=\phi(\hat{g}\cdot g , x),\forall g.\hat{g}\in G, x\in \mathcal{X}$, thus inducing families of smooth diffeomorphisms $\phi_g(x):=\phi(g,x)$. A group action is \textit{free} if $\forall x \in \mathcal{X},\phi(g,x)=x \Leftrightarrow g=e $ and \textit{transitive} if $\forall x,y \in \mathcal{X} \,,\,\exists g\in G$ such that $\phi(g,x)=y$ (i.e. the nonlinear smooth projections $\phi_x(g):=\phi(g,x)$ are surjective). If the group action is not free, a stabilizer exists, defined as $H_{\phi}(x):=\{g \in G\,|\,\phi(g,x)=x\} \subset G\,,\forall x\in\mathcal{X}$. A \textit{homogeneous} space is a smooth manifold $\mathcal{X}$ that admits a transitive group action $\phi: G \times \mathcal{X} \rightarrow \mathcal{X}$ and the Lie group $G$ is, then, called the \textit{symmetry} of $\mathcal{X}$. The group torsor $\mathfrak{G}$ of a Lie group $G$ is defined as the underlying manifold of $G$ without the group structure, allowing for identification of the torsor elements by the group elements, denoted $\chi\in \mathfrak{G} \simeq g \in G$, and inheriting the free and transitive group action $\phi$ induced by the group operator, i.e. for $\hat{g}\in G$ and $\chi\in \mathfrak{G} \simeq g \in G$ it stands that $\phi(\hat{g},\chi) \simeq \hat{g}\cdot g$. Crucially, a manifold that serves as a torsor for multiple Lie groups may admit multiple symmetries.

\subsubsection{Mechanics on manifolds \& Lie Groups}
    Consider a homogeneous swarm comprised of N rigid-body agents with position $\mathbf{p}_i\in \mathbb{R}_i^3$, orientation $\mathbf{R}\in SO(3)$, i.e. $\mathbf{R}_i^T \mathbf{R}_i =I \wedge det(\mathbf{R}_i)=1$, linear body-frame velocity $\mathbf{v}_i\in \mathbb{R}^3$ and angular body-frame velocity $\mathbf{\omega}_i\in \mathbb{R}^3$, for $i \in I_N=[1,...,N]$. The tensor bundle $q_i=[\mathbf{p}_i^T, vec(\mathbf{R}_i)^T] \in Q\equiv SE(3)$ denote the generalized coordinates of  and $\zeta_i = [\mathbf{v_i}^T,\mathbf{\omega}_i^T]\in \mathcal{T}_{q_i}Q \equiv\mathbb{R}^6$ the generalized velocity each robot. Let $\hat{p}_i=M(q_i)\zeta_i \in \mathbb{R}^6$ denote the generalized momentum, with $M:Q \rightarrow \mathbb{R}^6$ positive-definite generalized mass matrix, and $x_i=(q_i,\hat{p}_i)\in \mathcal{T}^{*}Q$ the state of the robot on the cotangent tensor bundle of the $Q$ differentiable smooth manifold. The energy landscape of each robot is, then, described by the Hamiltonian (Legendre transform of the Lagrangian) $\mathcal{H}_i(q_i,p_i)=\mathcal{K}(q_i,p_i)+\mathcal{V}(q_i)\,,\, i \in I_N$, where $K:Q\times \mathbb{R}^6 \rightarrow \mathbb{R}$ the kinetic energy and $\mathcal{V}:\mathbb{R}^6 \rightarrow \mathbb{R}$ the potential energy of the robot. Assuming quadratic kinetic energy function $\mathcal{K}(q_i,p_i)= \frac{1}{2}p_i^T M(q_i)p_i$, the robot motion dynamics are described by the autonomous tensor field bundle $\dot{x}_i(t)=f(x_i(t),u_i(t))\,,\, i\in I_N$, with $x_i(t_0)=x_{i,0}\,,\, x_i\in \mathcal{X} \equiv \mathcal{T}^{*}Q$ and constrained actions $u_i\in \mathcal{U}$. The Hamiltonian dynamics can be further extended to include energy dissipation. Assuming that a configuration space that consists a group torsor for a Lie group and that the system dynamics extracted from the Hamiltonian have a symmetry on that Lie group, the degrees of freedom may be reduced, allowing for reduced computational demands and elimination of singularities by operating on coordinate-free frames in the associated Lie algebra, as exhibited in \cite{duong2024port, 8550238}.










\subsection{Problem Statement}\label{problem_statement}
Consider a homogeneous multi-robot dynamical system, comprising of $N$ autonomous robots indexed $i\in \{1,\dots,N\} \equiv I_N$. Let $\mathcal{X}$ be a smooth manifold and $\mathcal{U}$ a finite dimensional input space. The agents are described by dynamics:
\begin{align}
    \dot{x}_i(t) = f(x_i(t),u_i(t)),\quad x_i(0)=x_{i}^0,\forall i\in I_N
\end{align}
where $u_i\in \mathcal{U},x_i\in\mathcal{X}$ and $f:\mathcal{X}\times \mathcal{U} \rightarrow \mathfrak{X}(\mathcal{X})$ a linear morphism. Consider a Lie group $G$ and a smooth transitive group action $\phi:G \times \mathcal{X}\rightarrow \mathcal{X}$. The lift of the system $\Lambda:\mathcal{X}\times \mathcal{U}\rightarrow \mathfrak{g}$ is a smooth function that satisfies $d\phi(\Lambda(x_i(t),u_i(t)),x_i(t))= f(x_i(t),u_i(t))$. The lift provides the structure for a representaion of the system on the symmetry Lie group $\dot{g}_i(t) = dR_{g_i(t)} \Lambda(\phi(g_i(t),\Bar{x}),u_i(t))$, where $g_i(t)\in G$ with initial conditions $\phi(g_i(0),\Bar{x})=x_{i}^0$ and $\Bar{x}\in\mathcal{X}$ the origin point for the global coordinate parametrization. The transitivity of the group action is required for the projection maps $\phi(\cdot,x),\forall x\in \mathcal{X}$ to be surjective, guaranteeing the existence of a lift (since $\Lambda(x_i(t),u_i(t)) = d\phi^{\dagger}(e,x_i(t))f(x_i(t),u_i(t))$ is a valid lift \cite{9303761}). If the action is, also, free, the lift is unique. The trajectory of the dynamical system may be recovered from the trajectory of lifted system, evolving in the Lie group by the group action $x_i(t) = \phi(g_i(t),\Bar{x})$. That is because, assuming $g_i(t)$ a solution of the lifted system and $\phi(g_i(0),\Bar{x})=x_i(0)$, it stands that $\dot{x}_i(t)=d\phi(\dot{g}_i(t),\Bar{x})=d\phi(\Lambda(x_i(t),u_i(t)),x_i(t))=f(x_i(t),u_i(t))$ and, thus, via uniqueness of solutions of differential equations $x_i(t) = \phi(g_i(t),\Bar{x})$. Furthermore, if $\mathcal{X}\equiv \mathfrak{G}$, where $\mathfrak{G}$ the torsor of $G$, the manifold inherits a transitive and free action from the group $G$ and, for $\Bar{x}=e$, all elements of the torsor are identified by elements of the group, leading to $\Lambda(g_i(t),u_i(t))=dR_{g_i(t)}f(x_i(t),u_i(t))$ with $g_i(t)\simeq x_i(t)$ \cite{HAMPSEY2023132}.

\noindent \textbf{Graph Representation of Multi-robot Systems}\label{intro:graph_representation}: We assume that the robots are equipped with sensing/communication capabilities with a range $\hat{\epsilon}$. Let $\mathcal{N}_i:= \{j\in I_N \setminus\{i\} \,:\, d(x_i,x_j)\leq \hat{\epsilon} \}\,,\, \forall i \in I_N$ denote the neighbourhoods, thus giving rise to a graph representation of the system $\mathcal{G}_t=\{V
_{\mathcal{G}_t},\mathcal{E}_{\mathcal{G}_t}\}$, with nodes $V
_{\mathcal{G}_t}=\{x_i(t)\,,\, i\in I_N\}$ and edges $\mathcal{E}_{\mathcal{G}_t}=\{ (i,j)\,,\, : \forall i\in I_N,j\in \mathcal{N}_i \}$. Information is propagated over the graph structure, with each robot receiving local observations of the system, denoted $o_i(t)=\{x_j(t)\,,\, j\in \mathcal{N}_i\}\,,\, i\in I_N$. We denote $x(t)=[\oplus_{\forall i\in I_N} x_i(t)]\in \cup_{i\in I_N}\mathcal{X}$ and $u(t)=[\oplus_{\forall i\in I_N} u_i(t)]\in \cup_{i\in I_N}\mathcal{U}$ the centralized state and action of the multi-robot system respectively. Assuming that a submanifold $\Bar{X} \subseteq\mathcal{X}$ forms the torsor $\mathfrak{G}$ of the Lie group $G$ and that $\mathcal{X}\setminus \Bar{X}$ is compatible with $G$, then every robot inherits a group representation element $g_i\,,\forall i\in I_N$ and the node attributes of the graph become $V_{\mathcal{G}_t}=\{(g_i(t),x_i(t))\,,\, i\in I_N\}$.
 
\noindent \textbf{Problem statement}: Given a swarm of $N$ robots of known dynamics, the trajectories $\{x_i(t)\,,\, i\in I_N\},t\in \mathbb{R}^{+}$ evolve in a complex environment, known or estimated continuously through onboard sensors, with obstacles represented as a point cloud set $\mathcal{O}\in \mathbb{R}^{3 \times d}$. Assuming a metric function denoted $\mathcal{L}: \cup_{i\in I_N} \mathcal{X} \times \cup_{i\in I_N} \mathcal{U} \rightarrow \mathbb{R}$ that codifies the specific task (e.g. distance for navigation, alignment for flocking), we formally define the multi-agent geometric optimization problem
\begin{align}
\label{eq:prob}
    u^{*}_{0:T,I_N}=& \argmin_{u_{0:T}} \int_{0}^T \mathcal{L}(\oplus_{I_N}x_i(\tau), \oplus_{I_N}u_i(\tau)) d\tau \nonumber\\
    s.t.\quad& \dot{x}_i(t)=f(x_i(t),u_i(t))\in \mathfrak{X}(\mathcal{X})\,,\, i\in I_N \nonumber\\
    &u_i(t) = \pi(o_i(t) \cup x_i(t);\mathcal{O}) \in \mathcal{U}
\end{align}
Problem (\ref{eq:prob}) amounts to $N$ robots learning the distributed control policy $\pi_\theta: \cup_{\mathcal{N}_i \cup \{i\}} \mathcal{X} \times \mathbb{R}^{3 \times d} \rightarrow \mathcal{U} $ using only local observations and knowledge of the environment. This problem can be recast as a distributed Multi-Agent Reinforcement Learning problem by maximizing a reward function instead of minimizing a loss function, with robot dynamics described by a transition function, thus forming an MDP. For clarity reasons we use the optimal control jargon.




==> Extended_version_files/SE3_Transformer_extended.tex <==
\section{Equivariant Graphormer}\label{section:LieGraphormer}
To solve the Geometric Swarming problem described in Section \ref{problem_statement}, we must learn the distributed equivariant policy $\hat{u}_i(t)=\hat{\pi}(o_i \cup x_i;\mathcal{O}) \,,\, i\in I_N$, as described in Section \ref{}. Generally deep learning models require specialized architectures to ensure the satisfaction of the equivariant constraints \cite{}. Such architectures can result in more challenging optimization \cite{} that can complicate their integration with standard Reinforcement Learning techniques. To address these challenges we proposed to leverage the structure of our input graph representation and achieve equivariance through group canonicalization, described in Section \ref{sec:groupcanon}. This technique doesn't impose any additional constrains to the model architecture and thus it allows us to easily extend pre-existing arcitectures used by previous work to learn distributed swarming policies.  To that end, in Section \ref{sec:equivgraphTransformer} we describe an equivariant extension of the Graph Transformer \cite{müller2023attending}. 
\subsection{Group Canonicalization}\label{sec:groupcanon}
Given a group $G$ acting on space $X$ through action $\phi_g$ we can define an extended group action $\phi'_g$ on space $G\times X$ as:
\begin{equation}
    \phi'_g[(p,x)]=(g\cdot p,\phi_g[x]),\quad \forall g,p\in G, x\in X
\end{equation}
here it is easy to see that since $\phi_g$ is an action of group $G$, $\phi'_g$ satisfies the properties of definition \ref{definitioin:group_action} and thus it is also an action.
\par  Now assume an additional output space $Y$ with $\psi_g:G\times Y\to Y$ being the corresponding group action for all $g\in G$. We can leverage the special structure of a function $f:G\times X\to Y$ to show the following:
\begin{lemma_}\label{lem:canonic}
A function $f:G\times X\to Y$ satisfies the equivariant constraint $f(\phi'_g[p])=\psi_g[f(p)]$, $\forall g\in G$ and $p\in G\times X$, if and only if it can be written as a composition:
\begin{align*}
    f(g,x)=\psi_g[h(\phi_{g^{-1}}[x])],\quad \forall g\in G, x\in X
\end{align*}
with $h:X\to Y$ being equal to $h(x)=f(e,x)$ for all $x\in X$, with $e$ being the identity element of $G$.
\end{lemma_}
\begin{proof} We append the proof in Appendix I Section \ref{appendix:proofs} of the supplementary material.
\end{proof}
Notice that in Lemma \ref{lem:canonic}, $h$ is a function from $X$ to $Y$ without any additional constraints. This implies that we can use any general function approximator (e.g. MLP, Transformer) to approximate an equivariant function $f:G\times X\to Y$, by only applying the appropriate input-output transformations. We will use this observation to extend the baseline non-equivariant models to be equivariant with minimal changes to the underlying architecture.
\subsection{Equivariant Graph Transformer}\label{sec:equivgraphTransformer}
 Given a feature augmented graph representation $(V,E,F)$ with a finite set of nodes $V$, a finite set of edges $E(G)\subset \{(u,v)|u,v\in V\}$ and a set of per-node features $F=\{f_v\in X|v\in V\}$, a graph transformer sequentially updates the nodes features using a local attention layer to aggregate information from neighboring nodes. Specifically the $l^{th}$ update layer for node $v\in V$ is a function $M_v: X^{(l)}\to X^{(l+1)}$ defined as $f_v^{(l+1)}\leftarrow M_v(F^{(l)})=\mu(f_v^{(l)}+\mathrm{attn}(F^{(l)})_v)$, where $\mu$ corresponds to a fully-connected feedforward network, and $\mathrm{attn}$ corresponds to the local attention layer:
\begin{align*}
    \mathrm{attn}(F^{(l)})_v=\sum_{p\in \mathcal{N}_v}\frac{\mathrm{exp}\left(f_v^{(l)}^T W_Q^T W_Kf_p^{(l)}\right)}{\sum_{p\in \mathcal{N}_v}\mathrm{exp}\left(f_v^{(l)}^T W_Q^T W_K f_p^{(l)}\right)}\left(W_V f_p^{(l)}\right)
\end{align*}
with $\mathcal{N}_v$ being the set of neighbors for nodes $v$.
\par As discussed in Section \ref{intro:graph_representation}, in the case of the distributed swarming policy the input graph representation has an additional structure that enables to easily extend the graph transformer to be equivariant. Specifically, each node $v\in V$ additional to a feature $f_v\in X$ describing each state is also equipped with a local frame $g_v\in G$. This means that the input graph is represented  as $(V,E,F_\mathrm{tens})$, with $F_\mathrm{tens}=\{(g_v,f_v)\in G\times X|v\in V\}$ being a set of "tensorial" features that are described by their local frame $g_v\in G$ along with their feature value $f_v$. For such a feature $(g_v,f_v)$ expressed in local frame $g_v\in G$ we can compute the equivalent feature expressed in a new frame $g_n\in G$ by applying the action $\phi'_{g_ng_v^{-1}}[(g_v,f_v)]=(g_n,\phi_{g_ng_v^{-1}}[f_v])$. This structure allows us to leverage the results of Lemma \ref{lem:canonic} and define an equivariant update rule $M^\mathrm{eq}_v:G\times X^{(l)}\to X^{(l+1)} $ for the features of node $v\in V$ as follows:
\begin{align*}
    f_v^{(l+1)}\leftarrow M^\mathrm{eq}_v(g_v,F^{(l)})=\phi^{(l+1)}_{g_v}\left[M_v\left(\phi^{(l)}_{g_v^{-1}}\left[F^{(l)}\right]\right)\right]
\end{align*}
with $\phi^{(l)}, \phi^{(l+1)}$ being actions of group $G$ on the corresponding input/ouput feature space $X^{(l)}, X^{(l+1)}$. By sequentially composing the equivariant update layers we  define an end-to-end Equivariant Graphomer, which is used to learn the equivariant policy $\hat{\pi}$.
 

\begin{remark}(Robustness Characteristics)
    The Lipschitz constant of neural networks is directly connected to their robustness and adversarial vulnerability. The Group Equivariant Graphormer is by construction similar to any attention GNN, adjusted for group actions, and thus any Lipschitz-bounding scheme, e.g. spectral normalization \cite{pmlr-v139-dasoulas21a}, is directly applicable. As this is outside the scope of this paper, we leave that for future work.
\end{remark} 




==> files/Multi-agent_RL.tex <==
\section{DISTRIBUTED TRAINING}
...



\subsection{Imitation Learning}...
\subsection{Architecture}...
\subsubsection{Model efficiency}...



==> files/Problem_formulation.tex <==









\subsection{Problem Statement}\label{problem_statement}
Consider a homogeneous multi-robot dynamical system, comprising of $N$ autonomous robots indexed $i\in \{1,\dots,N\} \equiv I_N$. Let $\mathcal{X}$ be a smooth manifold and $\mathcal{U}$ a finite dimensional input space. The agents are described by dynamics:
\begin{align}
    \dot{x}_i(t) = f(x_i(t),u_i(t)),\quad x_i(0)=x_{i}^0,\forall i\in I_N
\end{align}
where $u_i\in \mathcal{U},x_i\in\mathcal{X}$ and $f:\mathcal{X}\times \mathcal{U} \rightarrow \mathfrak{X}(\mathcal{X})$ a linear morphism. Consider a Lie group $G$ and a smooth transitive group action $\phi:G \times \mathcal{X}\rightarrow \mathcal{X}$. The lift of the system $\Lambda:\mathcal{X}\times \mathcal{U}\rightarrow \mathfrak{g}$ is a smooth function that satisfies $d\phi(\Lambda(x_i(t),u_i(t)),x_i(t))= f(x_i(t),u_i(t))$. The lift provides the structure for a representaion of the system on the symmetry Lie group $\dot{g}_i(t) = dR_{g_i(t)} \Lambda(\phi(g_i(t),\Bar{x}),u_i(t))$, where $g_i(t)\in G$ with initial conditions $\phi(g_i(0),\Bar{x})=x_{i}^0$ and $\Bar{x}\in\mathcal{X}$ the origin point for the global coordinate parametrization. The transitivity of the group action is required for the projection maps $\phi(\cdot,x),\forall x\in \mathcal{X}$ to be surjective, guaranteeing the existence of a lift (since $\Lambda(x_i(t),u_i(t)) = d\phi^{\dagger}(e,x_i(t))f(x_i(t),u_i(t))$ is a valid lift \cite{9303761}). If the action is, also, free, the lift is unique. The trajectory of the dynamical system may be recovered from the trajectory of lifted system, evolving in the Lie group by the group action $x_i(t) = \phi(g_i(t),\Bar{x})$. That is because, assuming $g_i(t)$ a solution of the lifted system and $\phi(g_i(0),\Bar{x})=x_i(0)$, it stands that $\dot{x}_i(t)=d\phi(\dot{g}_i(t),\Bar{x})=d\phi(\Lambda(x_i(t),u_i(t)),x_i(t))=f(x_i(t),u_i(t))$ and, thus, via uniqueness of solutions of differential equations $x_i(t) = \phi(g_i(t),\Bar{x})$. Furthermore, if $\mathcal{X}\equiv \mathfrak{G}$, where $\mathfrak{G}$ the torsor of $G$, the manifold inherits a transitive and free action from the group $G$ and, for $\Bar{x}=e$, all elements of the torsor are identified by elements of the group, leading to $\Lambda(g_i(t),u_i(t))=dR_{g_i(t)}f(x_i(t),u_i(t))$ with $g_i(t)\simeq x_i(t)$ \cite{HAMPSEY2023132}.

\noindent \textbf{Graph Representation of Multi-robot Systems}\label{intro:graph_representation}: We assume that the robots are equipped with sensing/communication capabilities with a range $\hat{\epsilon}$. Let $\mathcal{N}_i:= \{j\in I_N \setminus\{i\} \,:\, d(x_i,x_j)\leq \hat{\epsilon} \}\,,\, \forall i \in I_N$ denote the neighbourhoods, thus giving rise to a graph representation of the system $\mathcal{G}_t=\{V
_{\mathcal{G}_t},\mathcal{E}_{\mathcal{G}_t}\}$, with nodes $V
_{\mathcal{G}_t}=\{x_i(t)\,,\, i\in I_N\}$ and edges $\mathcal{E}_{\mathcal{G}_t}=\{ (i,j)\,,\, : \forall i\in I_N,j\in \mathcal{N}_i \}$. Information is propagated over the graph structure, with each robot receiving local observations of the system, denoted $o_i(t)=\{x_j(t)\,,\, j\in \mathcal{N}_i\}\,,\, i\in I_N$. We denote $x(t)=[\oplus_{\forall i\in I_N} x_i(t)]\in \cup_{i\in I_N}\mathcal{X}$ and $u(t)=[\oplus_{\forall i\in I_N} u_i(t)]\in \cup_{i\in I_N}\mathcal{U}$ the centralized state and action of the multi-robot system respectively. Assuming that a submanifold $\Bar{X} \subseteq\mathcal{X}$ forms the torsor $\mathfrak{G}$ of the Lie group $G$ and that $\mathcal{X}\setminus \Bar{X}$ is compatible with $G$, then every robot inherits a group representation element $g_i\,,\forall i\in I_N$ and the node attributes of the graph become $V_{\mathcal{G}_t}=\{(g_i(t),x_i(t))\,,\, i\in I_N\}$.
 
\noindent \textbf{Problem statement}: Given a swarm of $N$ robots of known dynamics, the trajectories $\{x_i(t)\,,\, i\in I_N\},t\in \mathbb{R}^{+}$ evolve in a complex environment, known or estimated continuously through onboard sensors, with obstacles represented as a point cloud set $\mathcal{O}\in \mathbb{R}^{3 \times d}$. Assuming a metric function denoted $\mathcal{L}: \cup_{i\in I_N} \mathcal{X} \times \cup_{i\in I_N} \mathcal{U} \rightarrow \mathbb{R}$ that codifies the specific task (e.g. distance for navigation, alignment for flocking), we formally define the multi-agent geometric optimization problem
\begin{align}
\label{eq:prob}
    u^{*}_{0:T,I_N}=& \argmin_{u_{0:T}} \int_{0}^T \mathcal{L}(\oplus_{I_N}x_i(\tau), \oplus_{I_N}u_i(\tau)) d\tau \nonumber\\
    s.t.\quad& \dot{x}_i(t)=f(x_i(t),u_i(t))\in \mathfrak{X}(\mathcal{X})\,,\, i\in I_N \nonumber\\
    &u_i(t) = \pi(o_i(t) \cup x_i(t);\mathcal{O}) \in \mathcal{U}
\end{align}
Problem (\ref{eq:prob}) amounts to $N$ robots learning the distributed control policy $\pi_\theta: \cup_{\mathcal{N}_i \cup \{i\}} \mathcal{X} \times \mathbb{R}^{3 \times d} \rightarrow \mathcal{U} $ using only local observations and knowledge of the environment. This problem can be recast as a distributed Multi-Agent Reinforcement Learning problem by maximizing a reward function instead of minimizing a loss function, with robot dynamics described by a transition function, thus forming an MDP. For clarity reasons we use the optimal control jargon.



